Exploring the mechanisms of transverse relaxation of copper(II)-phthalocyanine spin qubits

Molecular spin qubits are promising candidates for quantum technologies, but their performance is limited by decoherence arising from diverse mechanisms. The complexity of the environment makes it challenging to identify the main source of noise and target it for mitigation. Here we present a systematic experimental and theoretical framework for analyzing the mechanisms of transverse relaxation in copper(II) phthalocyanine (CuPc) diluted into diamagnetic phthalocyanine hosts. Using pulsed EPR spectroscopy together with first-principles cluster correlation expansion simulations, we quantitatively separate the contributions from hyperfine-coupled nuclear spins, spin--lattice relaxation, and electron--electron dipolar interactions. Our detailed modeling shows that both strongly and weakly coupled nuclei contribute negligibly to $T_2$, while longitudinal dipolar interactions with electronic spins, through instantaneous and spectral diffusion, constitute the main decoherence channel even at moderate spin densities. This conclusion is validated by direct comparison between simulated spin-echo dynamics and experimental data. By providing a robust modeling and experimental approach, our work identifies favorable values of the electron spin density for quantum applications, and provides a transferable methodology for predicting ensemble coherence times. These insights will guide the design and optimization of molecular spin qubits for scalable quantum devices.

==> Latest_version_CuPc_EPR/ElectronSpinBath.tex <==
\begin{figure}[htbp]
\includegraphics[width=0.46\textwidth]{Latest_version_CuPcEPR_Figure/CuPcEPR_fig4v4.pdf}
\caption{\textbf{CCE results and electron--electron spin interaction effects.} The $T_2$ decay rates obtained from CCE simulations are shown as gray (CuPc:NiPc) and purple (CuPc:H$_2$Pc) curves, at varying CuPc doping percentages. The black dashed line represents the simulated total decoherence rate from electron spin bath interactions, incorporating \textit{flip-flop interactions}, \textit{instantaneous diffusion}, and \textit{spectral diffusion} discussed in Section.~\ref{section:electron}. Experimental data measured at doping ratios of CuPc:NiPc = 1:140 and CuPc:H$_2$Pc = 1:45 are also plotted, showing good agreement with the simulated overall electron spin bath effect.
\label{fig:4}}
\end{figure}

\section{Electron Spin Environment\label{section:electron}}
Although much less dense, electronic spins
can greatly contribute to decoherence, due to their stronger interactions. 
%As mentioned in the introduction section, for solid state qubits like NV center, the electron-electron interaction is an important decoherence source. 
In an CuPc:XPc crystal, the electron spin bath predominately consists of the electron spins from all the other CuPc spins~\cite{warner2013potential,sushkov2014magnetic,escalera2019decoherence}, giving rise to a complex many-body system.

Despite the apparent lack of distinction between ``system'' and ``environment'', we can still consider how a probe CuPc \textit{central} spin  is  %This interaction can still be analytically modeled as  and 
affected by a spin bath consisting of the other CuPc molecules. According to the simulation of the the dynamics in a single molecule in Section.~\ref{section:mechanics}, where the strongly coupled nuclear spins ($Cu$, $N$) are effectively frozen and only contribute to frequency shift.
In particular, we can treat the nuclear spins as classical (and frozen) and 
we can focus on a central effective spin-\(1/2\) (representing the spin packet that is resonantly driven in the spin echo sequence, labeled by \(\iota_R\)) coupled to a bath of electronic spins each with their effective frequency $\Delta_\iota$, 

%where each containing all of its effective spin-\(1/2\) transitions. 
% \begin{equation}
% \begin{aligned}
%    H_e =\ & \Delta_{\iota_R} S_z^{\iota_R} + \sum_k^N \vec{S}^{\iota_R} \cdot \mathbf{D}^k \cdot \bigoplus_{\iota}^M \vec{S}^{k,\iota} \\
%    & + \sum_k^N \bigoplus_{\iota}^M \left( \Delta_{\iota} S_z^{k,\iota} + \sum_{k'}^N \bigoplus_{\iota'}^M \vec{S}^{k',\iota'} \cdot \mathbf{D}^{k'k} \cdot \vec{S}^{k,\iota} \right),
% \end{aligned}
% \label{eq:hamilton_electronspin_initial}
% \end{equation}
% where \(k\) indexes CuPc molecule, \(N\) denotes the total number of CuPc molecule. $\mathbf{D}$ is the electron-electron spin dipolar interaction coefficient which can be calculated numerically. The last term describes the interactions among the bath spins. 

% Additionally, it is reasonable to assume that the electron spin spin bath is initially in a fully mixed state at cryogenic temperatures, as the thermal polarization of the electron spins under the experimental condition remains negligible.
%--the population is near equally distribution among all the energy levels. 


%Given these considerations, it can be shown that, under ensemble averaging, rather than explicitly modeling all hyperfine sublevels of every molecule (Eq.~\eqref{eq:hamilton_electronspin_initial}), the spin bath can be effectively simplified by assigning each CuPc site only with only one electron spin-1/2, whose transition frequency is stochastically sampled from the hyperfine-shifted frequencies. Ensemble averaging is required by repeatedly resampling these transition frequencies. A rigorous analytical calculation justifying this equivalence is provided in the Appendix.~\ref{appendix:electron_spin_bath}.

The Hamiltonian for \(N\) electronic spins (\(N\) CuPc molecules within a finite volume) can be written as
%for each sampling can thus be written as:
\begin{equation}
\begin{aligned}
    {\cal H}_e' = &\ \Delta_{\iota_R} S_z^{\iota_R} + \sum_{k=1}^N \vec{S}^{\iota_R} \cdot \mathbf{D}^k \cdot \vec{S}^k \\
    &+ \sum_{k=1}^N \left( \Delta_{\iota_k} S_z^k + \sum_{k'=1}^N \vec{S}^{k'} \cdot \mathbf{D}^{k'k} \cdot \vec{S}^k \right),
\end{aligned}
\label{eq:hamilton_electronspin_2}
\end{equation}
where \(k\) indexes individual electron spin sites each with frequency $\Delta_{\iota_k}$ set by the (random) nuclear spin state. %with \(N\)  the total number of electron spin sites, equivalent to the number of CuPc molecules within a finite volume. The resonance frequency of the effective spin at each site \(\omega_k\) is randomly sampled from\(\{\Delta_{\iota}\ |\iota = 1,\ldots,2M\}\).
We note that here are $2M$ nuclear spin packets because the $\beta$-phase CuPc-XPc crystal contains two distinct orientations of CuPc molecules in the lattice (illustrated as up-tilted and down-tilted columns in Figure~\ref{fig:1}), and each orientation exhibits a distinct set of \(M=36\) hyperfine-shifted spin-\(1/2\) transitions. Evolution under this Hamiltonian is then averaged over the CuPc  positions and the intra-molecule nuclear spin  states at thermal equilibrium.

 We note that due to the large Zeeman energy in the chosen magnetic field, the dipolar interaction $\vec{S}^{\iota_R}\cdot \mathbf{D}^k\cdot \vec{S}^k$ and $\vec{S}^{k'} \cdot \mathbf{D}^{k'k} \cdot \vec{S}^k$ in Eq.~\eqref{eq:hamilton_electronspin_2} reduces to its secular part with two distinct components, a transverse term \(D_{\perp}(S_xS_x + S_yS_y)\) and a longitudinal term $D_{zz}S_zS_z$. In the following, we  quantitatively investigate the coherence properties of the central spin under these components.
 %Previous studies~\cite{warner2013potential,escalera2019decoherence} inaccurately estimated the flip-flop contributions {\color{red}lower the tune?} to decoherence with an oversimplified  spin environment and the contribution from longitudinal interactions has not been fully captured in previous studies. 


\subsection{Flip-Flop Processes}
%
The transverse component of the magnetic dipolar interaction induces flip-flop processes. By using the standard ladder operators \(S_{\pm}\)  to rewrite  it,  (\(D_{\perp}(S_xS_x + S_yS_y)\equiv D_{\perp}(S_+S_- + S_-S_+)\)), makes it clear that this interaction drives transitions \(\ket{\uparrow\downarrow} \rightarrow \ket{\downarrow\uparrow}\) between spin pairs, leading to polarization transfer that causes decoherence.

The flip-flop rate between two  spins with  energy mismatch $\Delta$ and transverse coupling strength $D_{\perp}$ is
\begin{equation}
\Gamma_{\text{ff}}(\Delta) = \frac{D_{\perp}^2}{\sqrt{\Delta^2 + D_{\perp}^2}}.
\end{equation}
To evaluate the flip-flop effect we consider again a central probe spin interacting with a large bath of electronic spins in a thermal state. 
%where \(\delta\) is the energy mismatch between the central spin and bath spin, and \(|D_{\perp}|\) is the root-sum-square (RSS) of the dipolar coupling strength among the bath with spin density \(n_e\) as: $|D_{\perp}| = \frac{\mu_0}{4\pi} \gamma_e^2 \hbar \sqrt{\frac{8}{105}} n_e.$
The spin bath contains \(M\) equally populated  nuclear spin manifolds, setting the frequency of each electronic spin,  \(\Delta_{\iota}\). The total flip-flop rate experienced by the central spin is the sum of contributions from all of the M groups, 
\begin{equation}
\Gamma_{\mathrm{flip\text{-}flop}} 
= \sum_{\iota}  \frac{\langle D_{\perp,\iota}^2\rangle}{\sqrt{(\Delta_{\iota_R} - \Delta_{\iota})^2 + \langle D_{\perp,\iota}^2\rangle}},
\end{equation}
where $\langle D_{\perp,\iota}^2\rangle$ is second moment of the dipolar couplings of a bath with spin density \(n_e^\iota=n_e/M\): $\sqrt{\langle D_{\perp,\iota}^2\rangle} = \frac{\mu_0\hbar}{4\pi} \gamma_e^2  \sqrt{\frac{8}{105}} \frac{n_e}M$.
 The contribution of flip-flops  to the transverse relaxation rate can be approximated as 
%\begin{equation}
\(R_{\mathrm{flip\text{-}flop}} = \frac{1}{2} \Gamma_{\mathrm{flip\text{-}flop}}.\)
%\end{equation}
For CuPc:H\textsubscript{2}Pc at a 1:49 doping ratio and CuPc:NiPc at 1:140 we estimate $ \Gamma_{\mathrm{flip\text{-}flop}} \approx 0.11~\mathrm{MHz} $ and \(\approx 0.03~\mathrm{MHz}\), respectively, indicating that only spins from the same manifold as $\iota_R$ contribute. These values are significantly lower than the measured spin echo dephasing rates, which lie in the MHz range. 
%This allows to approximate simplification of our model in Eq.~\eqref{eq:hamilton_electronspin} that spin flips of the central spin can be neglected when modeling its coherence dynamics from the effects of longitudinal interactions ($D_{\parallel} S_z$), which will be discussed in detail in the following subsection.
These observations allow us to simplify our subsequent model for the electronic spin bath and focus on the effects of the longitudinal dipolar term. In doing so, we can assume that the central spin will not undergo a spin flip in the time it takes it to decohere due to the dipolar longitudinal term contribution. We remark that this small effect of the flip-flop can be attributed to the effective reduced density, $n_e/M$, of the spin bath that arises from the resolved nuclear spin manifolds.




\subsection{Dephasing from $S_z$ Interaction}

The longitudinal term in the dipolar interaction,   \(\sim~\!D_{\parallel} S_z\), contributes to dephasing and thus plays a crucial role in transverse decoherence. 
Its effects in spin echo experiments depends on whether the bath spins are themselves driven by %, depending on whether the environmental spins can be coherently driven into superposition states by 
the microwave pulses. Then we can describe the spin probe to be interacting with two distinct sets of CuPc spins: ``\textit{A} spins'', which  are driven by the control microwave field because their transition frequencies are near  resonance; and ``\textit{B} spins'', which are unaffected by the microwave excitation due to their energy detuning  due mostly to hyperfine interactions.   
$A$~spins give rise to instantaneous diffusion while $B$ spins to spectral diffusion, two distinct dephasing mechanism that   we analyze next.

\subsubsection{Instantaneous Diffusion Effect}

Instantaneous diffusion (ID)  arises from longitudinal dipolar interactions between spins that are simultaneously flipped by a microwave pulse, that is,  $A$ spins. %In our case, this refers to the on resonant spins, i.e., the A spins as defined above. 
In a spin echo, the longitudinal coupling \(D_\parallel S_z S_z\) between two $A$ spins remains invariant under the  (resonant) \(\pi\)-pulse. 
%inverts all addressed spins simultaneously, the longitudinal interaction term between any two such spins, \(S_z S_z\), remains invariant under the transformation: $(-S_z)(-S_z) = S_z S_z$.
As a result,
%the dipolar field $D_{\parallel}S_z S_z$ experienced by each A spin (including central spin in our model) does not reverse after the pulse, so 
the phase accumulated due to $D_\parallel^k$ is not refocused and   results in incoherent dephasing among the $A$ spins.

While this is a large effect, not mitigated by the echo, it is somewhat alleviated by the effective smaller density of the $A$ spins, $n_e/M$. 
 Then, the instantaneous diffusion dephasing rate in  our CuPc:XPc samples can be quantitatively estimated to be
~\cite{schweiger2001principles}:
% \begin{equation}
%     R_{\mathrm{ID}} = \sum_{\iota=1}^M \frac{n_e}{M}\cdot \frac{4\pi^2}{9\sqrt{3}} \cdot \frac{\mu_0 \gamma_e^2 \hbar}{4\pi} \cdot \delta(\omega_\iota -\omega_{\mu w}).
% \end{equation}
\begin{equation}
    R_{\mathrm{ID}} = \frac{n_e}{M}\cdot \frac{4\pi^2}{9\sqrt{3}} \cdot \frac{\mu_0 \gamma_e^2 \hbar}{4\pi}.
\end{equation}
% The resonance condition \(\delta(\omega_\iota -\omega_{\mu w})\)  can be 
% %The summation is taken over all \(A\) spins that are resonant with the microwave. In practice, this resonance condition is 
% relaxed to a near-resonance criterion: \(|\omega_\iota - \omega_{\mathrm{\mu w}}| < \Omega_{\mathrm{\mu w}}\), where \(\Omega_{\mathrm{\mu w}}\) is the driving spectral width   due to  power broadening.
%, when spins with transition frequencies in the vicinity of \(\omega_{\mathrm{\mu w}}\) are also effectively excited.
This estimate yields \(R_{\mathrm{ID}} \approx 0.6\,\text{MHz}\) for CuPc:NiPc at a mixing ratio of 1:140, and \(R_{\mathrm{ID}} \approx 1.88\,\text{MHz}\) for CuPc:H\textsubscript{2}Pc at 1:49

%The effect of \(S_z S_{\perp}\) coupling between A spins are neglected. This interaction can induce spin flips in neighboring spins, which are strongly suppressed by energy conservation and are therefore negligible compared to the dephasing induced by the \(S_z S_z\) interactions discussed above. 
%However, this is not necessarily the case when considering interactions between on-resonant (A spins) and off-resonant spins (B spins). In that context, the \(\pi\)-pulse inverts the sign of the \(S_z\) operator of the A spins only, effectively refocusing the phase accumulation due to \(S_z S_z\) interactions with B spins that are not actively driven by the control field. However, because B spins can still evolve under their internal Hamiltonian during the spin echo sequence, this refocusing does not eliminate decoherence arising from \(S_z S_{\perp}\) terms, which can contribute to dephasing. In the next section, we evaluate the effect of interactions with off-resonant B spins in detail.

\subsubsection{Spectral Diffusion Effect}
The $A$-$B$ longitudinal dipolar interaction, $\sim~D_\parallel S_zS_z$, is ideally canceled by the spin echo $\pi$ pulse on the A spin. However, the B spin dynamics leads to imperfect cancellation. This dynamics changes the effective local field felt by the A spin, thus leading its frequency to ``diffuse'' during the evolution, which causes decoherence
%Spectral diffusion refers to the decoherence process where longitudinal or spin-spin relaxation of off-resonant bath spins (B spins) changes the local field at the A spins, which leads to a transfer of A spin magnetization or coherence to parts of the spectrum where spins cannot be excited or detected directly 
~\cite{schweiger2001principles}. 

%The Hamiltonian describing the central spin interacting with off-resonant bath spins with neglecting the transverse interaction terms on the central spin can be written as:
% \begin{equation}
% \begin{aligned}
%     {\cal H}_{e,A\text{-}B}' = &\,\Delta_{\iota_R} S_z^{\iota_R} + S_z^{\iota_R} \cdot \sum_k \sum_{\mu = x,y,z} D^k_{z\mu} \cdot S_\mu^k \\
%     &+ \sum_{k,\,\omega_k \ne \Delta_{\iota_R}} \left( \omega_k S_z^k + \sum_{k'} \vec{S}^{k'} \cdot \mathbf{D}^{k'k} \cdot \vec{S}^k \right).
% \end{aligned}
% \label{eq:hamilton_electronspin_3}
% \end{equation}
In contrast to the electron-nuclear spin interaction model, the dipolar interactions among bath spins ($B$ spins), see second line of Eq.~\ref{eq:hamilton_electronspin_2},  are of the same order of magnitude as the interactions between the central spin ($A$ spin) and the bath spins.
This fast dynamics 
%The dipolar interactions among B spins will 
contribute to the decoherence of the central spin during a spin echo sequence. 
%For example, an intuitive case is that a spin flip of a B spin, induced by its interaction with neighboring B spins, modifies the local magnetic environment at the central spin. This perturbation changes the accumulated phase of the central spin that is not fully refocused by the \(\pi\)-pulse.

To quantitatively evaluate the many-body dynamics governed by this Hamiltonian, we employ the cluster-correlation expansion (CCE) method for an electronic spin bath. For each simulation instance, bath spins are randomly placed at molecular sites of XPc within the $\beta$-phase CuPc:XPc crystal lattice in a finite simulation volume. Each site is assigned a transition frequency randomly drawn from the simulated hyperfine spectrum corresponding to its specific molecular orientation.

Spin echo dynamics is then simulated for each generated spin configuration. Ensemble averaging is performed by repeating the initialization of the bath over many realizations until convergence is reached. Since the experiment is conducted on a powder sample, the final simulated signal is obtained by averaging over all possible crystal orientations. Additional details regarding simulation parameters and convergence criteria are provided in the Supplementary Material.

The CCE simulation  yields a spectral diffusion-induced decoherence rate of \(R_{\mathrm{SD}} = 1~\mathrm{MHz}\) for CuPc:NiPc = 1:140 and \(R_{\mathrm{SD}} = 1.5~\mathrm{MHz}\) for CuPc:H\(_2\)Pc = 1:49. %Details of the simulation parameters and convergence criteria are provided in the Appendix and Supplementary Materials. 

By combining these results with the previously estimated contribution from A-A spin interactions (instantaneous diffusion), we obtain a complete prediction of the transverse decoherence rate as a function of CuPc:XPc doping ratio, as shown in Fig.~\ref{fig:4}. The predicted values agree well with experimental measurements, confirming that at these densities decoherence is dominated by the electron spin bath effects. 

Furthermore, the approximately linear dependence of the transverse decoherence rate on the CuPc concentration suggests that \(T_2^{-1}\) can serve as a metric for electron spin density across a wide doping range.

%Compared with the ID effect, where the A spins have a much less density than B spins, the effect of B spins is still weak, which thanks to the $\pi$-pulse that refocued the phase accumulation of the B spins. An intuitive classical picture to explain this is that the Z and X component of B spins generates fluctuating mangetic field at A spin since it is in a fully mixed state, which has a quasi-static and a AC-like component with frequency near the electron resonance frequency. The quasi-static component is effectively canceled by the $\pi$-pulse of the echo and the AC component accumulate much smaller phase due to the fast oscillation. This intuitive understanding is known as filter function, detailed discussed in appendix and SM.


==> Latest_version_CuPc_EPR/NuclearSpinBath.tex <==
\section{Nuclear Spin Environment\label{section:nuclear}}


As discussed, the $^{63/65}\mathrm{Cu}$ and four $^{14}\mathrm{N}$ nuclear spins adjacent to the Cu(II) center mainly induce frequency shifts and negligible ESEEM due to hyperfine interactions, but do not substantially contribute to the spin echo decay.
More far away nuclear spins, instead, are not quenched and induce decoherence. Their coupling strength to the electron spin sets the characteristics of two distinct  nuclear  spin baths~\cite{wang2024digital,hernandez2018noise, reinhard2012tuning,taminiau2012detection}. The closest nuclear spins  to the Cu(II) center form a \textit{quantum} spin bath, which must be described by the coherent evolution of the hybrid electron-nuclear spin system~\cite{bradley2019ten}. In contrast, weakly coupled nuclear spins, whose dynamics are largely independent of the electron spin state, constitute a \textit{classical} spin bath~\cite{pham2016nmr}, which can be modeled by a stochastic magnetic field, whose fluctuations are captured by their power spectral density. Further details of this model are provided in the Supplementary Materials.


%Therefore, analyzing the impact of $^{1}\mathrm{H}$ nuclear spins in H$_2$Pc and NiPc provides an estimate of the upper bound on decoherence contributions from nuclear spins within the host environment.

The $^{1}\mathrm{H}$ nuclei exhibit both stronger hyperfine couplings and higher abundance than other nuclear spin species in the lattice, and therefore constitute the dominant contributors to the quantum-classical spin bath. 
%Most of the $^{1}\mathrm{H}$ nuclear spins are from the protons at the periphery of the Pc molecules. 
In the H$_2$Pc matrix, the two additional protons located at the molecular center increase the overall $^{1}\mathrm{H}$ spin density by approximately 10\% compared to the NiPc matrix. Furthermore, the CuPc electron spin is  adjacent to the four center protons from two neighboring H$_2$Pc molecules (Fig.~\ref{fig:3}(b, c).) Comparing H$_2$Pc and NiPc can thus provide insights into the H spin role in decoherence. 


%In CuPc:XPc crystal, there are weakly coupled nuclear spins, including distant $^{14}\mathrm{N}$ and $^{1}\mathrm{H}$ nuclei within the CuPc molecule, as well as $^{63/65}\mathrm{Cu}$, $^{14}\mathrm{N}$, and $^{1}\mathrm{H}$ nuclei from nearby XPc molecules. Under the experimental condition, these nuclear spins are close to zero polarization and interact with the electron spin primarily via magnetic dipolar coupling, with negligible Fermi contact terms. Depending on their interaction strength, they may be categorized into a classical or quantum {\color{red}spin bath\cite{}.} Weakly coupled nuclear spins, whose evolution is unaffected by the electron spin state, generate a \textit{classical} stochastic magnetic field that can be described by its autocorrelation function or power spectral density. In contrast, strongly coupled nuclear spins form a \textit{quantum} spin bath as their evolution is significantly affected by the electronic spin dynamics; the back-action is thus best described by considering the coherent evolution of the hybrid electro-nuclear spin {\color{red}system~\cite{hernandez}. }

%Among all the surrounding nuclear spins, $^{1}\mathrm{H}$ dominates the spin environment due to their large gyromagnetic ratio and high natural abundance. 
%In the CuPc:XPc, we identified all nearby nuclear spin and calculated their hyperfine coupling with the Cu(II) electron spin, as detailed in the Appendix. $^{1}\mathrm{H}$ exhibit particularly strong hyperfine couplings and constitute the primary quantum spin bath. There are two main sources of strongly coupled $^{1}\mathrm{H}$ nuclei. The first are hydrogen atoms located at the periphery of XPc molecules adjacent to the CuPc molecule. The second arises when XPc is H$_2$Pc: in this case, two additional hydrogen atoms located at the molecular center introduce four more $^{1}\mathrm{H}$ nuclei two adjacent H$_2$Pcs, modifying the composition of the quantum spin bath. Importantly, given the geometric structure of the $\beta$-phase XPc lattice, the peripheral hydrogen atoms of adjacent molecules closer to the CuPc electron spin than those at the molecular center (of H$_2$Pc). Moreover, the presence of these additional hydrogen nuclei in H$_2$Pc increases the overall $^{1}\mathrm{H}$ spin density by approximately 12.5\% compared to NiPc. Studying the impact of $^{1}\mathrm{H}$ nuclear spins enables us to estimate an upper bound on the decoherence contributions from general nuclear spins present in the host matrix.


%This indicates a minor contribution from the central hydrogen nuclei of the XPc molecules to the electron spin dynamics, as we will further substantiate in the following text. More distant hydrogen atoms contribute primarily as a classical background field. 

We focus on a single on-resonance N-Cu manifold with frequency $\Delta_\iota$ and consider the reduced electron spin 
%Using the effective spin-1/2 model, the 
 Hamiltonian in the rotating frame  coupled to 
the hydrogen nuclear spin bath: 
\begin{align}
{\cal H}_n &={\cal H}_0+ {\cal H}_{e\text{-}n,q} + {\cal H}_{e\text{-}n,c}, \label{eq:hamilton_nuclearspin}
\end{align}
where the electron Hamiltonian ${\cal H}_0 = \delta_{\iota} S_z$ is set by $\delta_{\iota} = \Delta_{\iota_R} - \omega_{\mu w}$,  the detuning between the transition frequency $\Delta_{\iota_R}$ and the applied microwave frequency $\omega_{\mu w}$. 
The classical nuclear spin bath
\begin{align}
{\cal H}_{e\text{-}n,c} &= \gamma_e \tilde{B}_z(t) S_z\label{eq:hamiltonian_nc},
\end{align}
with $\gamma_e$  the gyromagnetic ratio of the electron, is described by   a time-dependent stochastic magnetic field, $\tilde{B}_z(t)$ generated by unpolarized hydrogen spins. The quantum component of the nuclear spin bath is given by
% \begin{align}
% {\cal H}_{e\text{-}n,q} &= \sum_{n} ( S_z \sum_{\sigma = x,y,z} A_{z\sigma}^{n} I_{\sigma}^{n} +  \gamma_H\vec{B}_0\cdot\vec{I}^{n} ), \label{eq:hamiltonian_nq}
% \end{align}
\begin{align}
{\cal H}_{e\text{-}n,q} &= \gamma_H{B}_0\sum_{n}I^n_z+ S_z \sum_{n}\sum_{\sigma = x,y,z} A_{z\sigma}^{n} I_{\sigma}^{n} , \label{eq:hamiltonian_nq}
\end{align}
where $\gamma_H$  is the hydrogen gyromagnetic ratio and $A_{z\sigma}^n$ is the hyperfine coupling tensor between the electron spin and the $n$-th $^{1}\mathrm{H}$ nuclear spin. At the experimental field $B_0 = 3545$~G the Larmor frequency is $\omega_H\approx15.09$~MHz.
%\omega_{\textrm{H}}
% \begin{figure*}[htbp]
% \includegraphics[width=1\textwidth]{Latest_version_CuPcEPR_Figure/CuPcEPR_fig3_v4_all.pdf}
% \caption{\textbf{Spin locking response of CuPc to quantum and classical hydrogen spin baths.} 
%  % (a) Spin locking pulse sequence: a $\pi/2$ pulse is followed by a continuous driving pulse (amplitude $\Omega_1$, duration $\tau$) phase-shifted by $90^\circ$, producing a static effective field along the $x$-axis in the rotating frame. 
%  %    (b) Schematic of the spin environment in $\beta$-phase H$_2$Pc: proximal hydrogen nuclei (purple) form a quantum spin bath via coherent coupling with the CuPc electron spin, while distant nuclei generate a classical fluctuating field (purple haze). 
%     (a) Spin locking (NOVEL) pulse sequence. The locking pulse acts as an effective static field along the x-axis in the rotating frame. (b--d) Experimental spin locking signal and fit for CuPc:H$_2$Pc and CuPc:NiPc at varying $\Omega_x$. 
%     (e--g) Simulated spin locking signal under a quantum  bath only of hydrogen spins, at the same $\Omega_x$ as in (b--d). 
%     (h,i) Oscillation amplitude $C_q$ (Eq.~\ref{eq:spinlockingfit}) as a quantum spin characteristic versus $\Omega_x$ for CuPc:H$_2$Pc and CuPc:NiPc from experiment (h) and simulation (i). 
%     (j,k) Oscillation frequency $\alpha'$ (Eq.~\ref{eq:spinlockingfit}) as second quantum spin characteristic versus $\Omega_x$ for the two matrices from experiment (j) and simulation (k). 
%     (l,m) Experiment data and Lorentzian fitting of classical bath characteristic $1/T_{1\rho}$ for CuPc:H$_2$Pc (l) and CuPc:NiPc(m) as a function of $\Omega_x$.}
% \label{fig:3}
% \end{figure*}

\begin{figure*}[htbp]
\includegraphics[width=1\textwidth]{Latest_version_CuPcEPR_Figure/CuPcEPR_fig3_v5.pdf}
\caption{\textbf{Spin locking response of CuPc to quantum and classical hydrogen spin baths.} 
    (a) Spin locking (NOVEL) pulse sequence. The locking pulse acts  as an effective static field along the x-axis in the rotating frame. 
    (b--c)Spatial distribution of $^1$H nuclear spins (purple dots) surrounding the CuPc electron spin (red dot with gray spin arrow), shown for %(b) CuPc:H$_2$Pc and (c) CuPc:NiPc crystals. 
     (b--d) Experimental spin locking signal and fit for CuPc:H$_2$Pc and CuPc:NiPc at varying $\Omega_x$. 
    (e--g) Simulated spin locking signal under a quantum bath only of hydrogen spins, at the same $\Omega_x$ as in (b--d). 
    (h-j) Signal oscillation amplitude $C_q$ and frequency $\alpha'$  (Eq.~\ref{eq:spinlockingfit}) as a function of $\Omega_x$ for CuPc:H$_2$Pc and CuPc:NiPc extracted from fits to the experimental data (circles) and from simulations (dashed lines.) 
    (l) Spin-locking classical decay rate $1/T_{1\rho}$ (Eq.~\ref{eq:P_classical_1}) CuPc:H$_2$Pc  and CuPc:NiPc(m) as a function of $\Omega_x$: Circles, wxperiment data; lines,   Lorentzian fitting.}
\label{fig:3}
\end{figure*}

%Due to the large energy mismatch between the electron Zeeman splitting, the hyperfine couplings, and the nuclear spin energies, longitudinal  interactions are retained while the transverse terms (e.g., $S_x$) are neglected.

To selectively probe the hydrogen nuclear spin bath, we performe a spin locking experiment~\cite{henstra1988nuclear,henstra1988nuclear}, whose sequence is shown in Fig.~\ref{fig:3} (a). The electron spin is first rotated to the x axis by a  $\pi/2$ $S_y$ pulse and then we apply a
%prepared in a superposition state $\ketbra{+}{+}$. 
%A 
continuous microwave drive at the same frequency with a 90$^\circ$ phase shift  to lock the electron spin. In the rotating frame (within the rotation wave approximation), the drive  Hamiltonian,
\[ {\cal H}_{\text{locking}} = \Omega_x S_x,\]
 is added to the system Hamiltonian in Eq.~\eqref{eq:hamilton_nuclearspin}.  This spin-locking field induces a dressed-state energy splitting of the electron spin $\Omega_r=\sqrt{\Omega_x^2+\delta_\iota^2}$, which protects against decoherence while enabling resonant polarization transfer to nuclear spins when this splitting matches the nuclear Larmor frequency. This protocol --also known as  Nuclear Orientation Via Electron Spin Locking (NOVEL)-- thus enables probing the environmental proton spins as done in quantum noise spectroscopy~\cite{suter2016colloquium,cywinski2014dynamical,yan2013rotating}.  

The spin coherence as a function of the the spin locking pulse duration is shown in Fig.~\ref{fig:3}(d--f) for exemplary driving strengths. When varying the driving strength $\Omega_x$, the electron spin  decoherence rate  reaches a maximum at the resonant condition $\Omega_r\sim\omega_H=15.09$~MHz. (See additional experimental results in the Supplementary Material).
% In addition, the observed decay profile exhibits two distinct components: a fast, damped oscillation within the first 2~$\mu$s, followed by a slower exponential decay tail, which we will show below that is attributed by the quantum and classical spin bath respectively.
% %The former indicates coherent polarization exchange between the electron spin and the surrounding quantum spin bath.
We observe two distinct components: a fast, damped oscillation within the first 2~$\mu$s and a slower exponential decay tail. 
We ascribe each feature to the  quantum and classical spin baths, respectively, as we can prove with a simple model and numerical simulations (Fig.~\ref{fig:3}(g--i)) 

%Numerical simulations of the spin dynamics under the interaction with a pure quantum spin bath reveal the same damped oscillations results, as shown in . 

The oscillation arises from coherent polarization exchange between the electron spin and the surrounding quantum spin bath. The presence  of multiple polarization transfer pathways between the electron spin and nuclear spins with varying coupling strength and ensemble averaging over all possible detuning $\delta_\iota$ and molecular orientations leads to a damping of the oscillations.  
We can reproduce the key features of the experimental oscillation, such as the frequency and damping rate, by simulating  the electron spin dynamics under the interaction with a pure quantum spin bath. The  electron spin polarization under coupling to a quantum spin bath is well described by :
\begin{equation}
    P_q(t) = (1 - C_q) - C_q e^{-\Gamma_q t} \cos(\alpha t),
    \label{eq:spinlockingfit}
\end{equation}
where $C_q$ denotes the polarization transfer amplitude, $\Gamma_q$ the damping rate , and $\alpha$  the oscillation frequency. A detailed analytical and numerical analysis of the spin-locking evolution is shown  in the Supplementary Material.

The slower decay tail, which is captured by a simple exponential  
\begin{equation}
    P_c(t) = e^{-t / T_{1\rho}},
    \label{eq:P_classical_1}
\end{equation}
arises from the classical spin bath~\cite{henstra2008theory,yan2013rotating,wang2020coherence} which sets the spin-locking relaxation time, $T_{1\rho} \propto \frac{2}{\gamma_e^2 S(\Omega_r)}$, to be proportional to the spectral density $S(\Omega_r)$ of the fluctuating magnetic field at the dressed-state splitting $\Omega_r$.

The total EPR signal after spin locking  thus includes both the quantum and classical contributions, 
%\begin{equation}
\(    P_{\mathrm{spin-locking}}(t) = P_q(t) \, P_c(t)\).
%\end{equation}
Fitting the data to this expression, we extract the relevant parameters %classical decoherence rate $1/T_{1\rho}$, the oscillation frequency $\alpha'$, and the polarization transfer amplitude $C_q$ from experimental fits at variant driving conditions, 
as shown in Fig.~\ref{fig:3}(j--l).

The fitted quantum spin bath parameters ($C_q$, $\alpha$) for H$_2$Pc and NiPc are nearly identical, consistent with the simulation results. The peak in $C_q$ and the dip in $\alpha$, corresponding to the maximum polarization transfer amplitude and the transfer rate, respectively, occur at the resonance condition  $\Omega_r\approx \omega_H$.

The spectral densities of the classical  hydrogen spin bath, given by $\gamma_e S(\omega) \propto  2 / T_{1\rho}$, are also similar in the two samples. H$_2$Pc exhibits a slightly higher peak amplitude (approximately 10\%) near the Larmor frequency, consistent with its higher hydrogen density.
The  linewidth of $S(\Omega_r)$ is on the order of 2~MHz, significantly broader than the intrinsic linewidth expected for a hydrogen nuclear spin bath, typically in the kilohertz range. This indicates that the $T_{1\rho}$'s linewidth is dominated by the inhomogeneous broadening of the EPR transitions, which  %In the presence of detuning $\delta_{\iota}$, the effective splitting of the dressed state of electron spin becomes $\Omega_r = \sqrt{\Omega_1^2 + \delta_{\iota}^2}$. In our experiment, the detuning $|\delta_{\iota}|$ 
can reach  8~MHz due to the $g$-factor anisotropy averaging in the powdered CuPc sample.
Due to the EPR transition broadening, the Hartmann-Hahn condition $\Omega_r = \omega_{\textrm{H}}$ is satisfied over a larger frequency range (here  %determined by the electron spin linewidth during the spin-locking period, leading to the observed NOVEL transfer profile with a width of 
approximately 2~MHz) as already observed 
%This broadening effect has been previously reported and attributed to the same origin 
in similar molecular systems~\cite{mathies2016pulsed,jain2017off}.

The results of the spin-locking experiments suggest that the additional hydrogen nuclear spins in the H$_2$Pc molecule have a minimal effect on  the combined quantum and classical spin bath. This observation also implies that other possible substitutions of the X molecule are also likely to have a limited impact on the spin bath composition. 

The spin-locking decay show that the role of the H in decoherence only becomes large in a relatively narrow range close to the resonance condition. We thus also expect that the H spin will not dominate the $T_2$ echo decay time (unless pulse spacings were close to the resonant condition, which is not the case in our experiments.)
Still, we cannot experimentally isolate the contribution of nuclear spins --and in particular hydrogen nuclear spins-- in the 
%So far, the influence of the hydrogen nuclear spin bath on 
spin echo ($T_2$) decoherence. We thus resort to numerical simulations using  the cluster correlation expansion (CCE) method~\cite{yang2008quantum,onizhuk2021pycce}.
We use the results obtained from spin locking measurements and modeling to incorporate  both quantum ($T_{n,\mathrm{qu}}$) and classical ($T_{n,\mathrm{cl}}$) components of the nuclear spin environment in the CCE model. 
%has not yet been discussed. The decay observed in spin-locking experiments is strongly influenced by inhomogeneous broadening of the EPR transitions, whereas this broadening does not affect spin echo measurements. 
%To evaluate the influence of the hydrogen nuclear spin bath on spin echo decoherence ($T_2$), we performed cluster correlation expansion (CCE) simulations incorporating both quantum ($T_{n,\mathrm{qu}}$) and classical ($T_{n,\mathrm{cl}}$) components of the nuclear spin environment (see Appendix for details on the CCE method)~\cite{yang2008quantum,onizhuk2021pycce}. 
By directly simulating the many-body dynamics (truncated to computationally accessible cluster sizes), CCE calculates   the total decoherence rate:
\[
\frac{1}{T_{n,\mathrm{cce}}} = \frac{1}{T_{n,\mathrm{qu}}} + \frac{1}{T_{n,\mathrm{cl}}}.
\]
The simulated decoherence rates due to nuclear spins for H$_2$Pc and NiPc are $T_{n,\mathrm{cce}}^{-1} = 90$~kHz and 80~kHz, respectively. These rates are significantly smaller than the experimentally observed echo decay rates $T_2^{-1}$, which lie in the MHz range. This discrepancy indicates that decoherence mechanisms beyond the nuclear spin bath contribute substantially to spin echo decay. Indeed, we do not expect a static (inhomogeneous) broadening of the linewidth to contribute to spin echo decay, since the $\pi$-pulse effectively refocuses static detuning effects. Spin echo $T_2$ measurements are instead  sensitive to dynamic fluctuations on the timescale of the echo duration.

Combining insights from both spin-locking experiments and CCE simulations, we conclude that the presence of additional hydrogen nuclear spins at the center of the XPc molecule does not significantly alter the nuclear spin environment. Furthermore, the nuclear spin bath contributes only a minor portion to the experimentally observed $T_2$ decoherence.
